Multi-block Bregman proximal alternating linearized minimization and its application to orthogonal nonnegative matrix factorization

We introduce and analyze BPALM and A-BPALM, two multi-block proximal alternating linearized minimization algorithms using Bregman distances for solving structured nonconvex problems. The objective function is the sum of a multi-block relatively smooth function (i.e., relatively smooth by fixing all the blocks except one) and block separable (nonsmooth) nonconvex functions. It turns out that the sequences generated by our algorithms are subsequentially convergent to critical points of the objective function, while they are globally convergent under KL inequality assumption. Further, the rate of convergence is further analyzed for functions satisfying the {\L}ojasiewicz's gradient inequality. We apply this framework to orthogonal nonnegative matrix factorization (ONMF) that satisfies all of our assumptions and the related subproblems are solved in closed forms, where some preliminary numerical results is reported.

==> TeX/Preamble.tex <==
\usepackage[%
	eqreset=section,
	thmreset=section,
]{myPreamble}
\usepackage{todonotes}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{multirow}
%\usepackage{authblk}
\makeatletter
\newcommand\mynum[1]{$ˆ{\@fnsymbol{#1}}$}
\makeatother
\CreateNewTheorem[Fact]{fact}[dummythm]{Fact}

% change operator font (default is bold)
% \makeatletter
%    \renewcommand\operator@font{\rm}
% \makeatother

% Notation for big vectors. Uncomment/change the command \bm to whatever you want
% \renewcommand\bm[1]{#1} % Removes bold face
% Usage: \bm{x}^k or simply \bm x^k

\newcommandx\p[3][1=\gamma,3=h]{\prox_{#1#2}^{#3}}

\newcommand\C{\mathcal C}
\makeatletter
	\newcommand\D[1][h]{%
		\@ifnextchar_{\operatorname D}{%
			\ifstrempty{#1}{\operatorname D}{\operatorname D_{#1}}%
		}
	}
	%
\makeatother
\newcommandx\FBE[2][1={f,g},2={\gamma h}]{\varphi_{#2}^{#1}}
\newcommandx\T[2][2={\nicefrac{h}{\gamma_i}},1={i }]{\operatorname T_{#2}^{#1}}
\newcommandx\M[2][2={\nicefrac{h}{\gamma}},1={ }]{\operatorname{\mathcal{M}}_{#2}^{#1}}
\newcommandx\TG[2][1={f,g},2={\gamma^k h}]{\operatorname T_{#2}^{#1}}
\newcommandx\RGH[2][1={f,g},2={\gamma h}]{\operatorname R_{#2}^{#1}}
\let\proj\relax
\DeclareMathOperator\proj{Proj}

%% Custom creferencing of BPALM
	\newcommand\refBPALM[1][ (\cref{alg:bpalm})]{%
		\hyperref[alg:bpalm]{{\sf BPALM}}#1%
	}%
	\newcommand\refaBPALM[1][ (\cref{alg:abpalm})]{%
		\hyperref[alg:abpalm]{{\sf A-BPALM}}#1%
	}%


==> TeX/Text/2.BPALM/Algorithm.tex <==
%We conclude this section by extending our setting of \refBPALM[] to the case with $q$ blocks of variables, i.e.,
% \begin{equation}\label{eq:multiBlockProb}
% 	\minimize_{x_1,\ldots,x_q\in\R^n}~~\varphi(x_1,\ldots,x_q)\equiv \sum_{i=1}^q f_i(x_i)+\phi(x_1,\ldots,x_q),
% \end{equation}
% in which for $i=1,\dots,q$ the following holds:
% \begin{enumeratass}
% 	\item\label{ass:basic:g1}%
% 		\(\func f_i{\R^m}{\Rinf\coloneqq\R\cup\set\infty}\) is proper and lower semicontinuous (lsc);
% 	\item\label{ass:basic:h1}%
% 		\(\func{h_i}{\R^m}{\Rinf}\) is strictly convex, \(1\)-coercive
% 		and essentially smooth;
% 	\item\label{ass:basic:f1}%
% 		\(\func{\phi}{\R^{n_1}\times\ldots \times\R^{n_q}}{\Rinf}\) is $\C^1(\interior\dom h_1\times\ldots \times \interior\dom h_q)$, $\phi(x_1,\ldots,x_{i-1},\cdot,x_{i+1},\ldots,x_q)$ is \DEF{\(L_i\)-smooth relative to \(h_i\)} (i.e., \(L_i h_i(\cdot)-\phi(x_1,\ldots,x_{i-1},\cdot,x_{i+1},\ldots,x_q)\) is convex);
% \end{enumeratass}

%For the problem \eqref{eq:P}, an extension of \refBPALM[] can be extended using the well-known Gauss–Seidel, which we present in the following.

%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm*}[ht] 
\algcaption{({\bf MB-BPALM}) Multi-block BPALM}%
\begin{algorithmic}[1]
\Require{%
	\(\gamma\in{\left]0,\nicefrac{1}{L_f}\right[}\),~$c_1>1$,~
	\(x^0\in\R^n\).%
}%
\Initialize{$k=0$.}%
\State\label{state:bpalmmXk1}%
	for $i=1,\ldots,q$, set $\gamma_{i,k}=\tfrac{1}{c_i L_i}$ and compute
	\begin{equation*}
	    x_i^{k+1}\in\argmin_{x\in\R^m}\set{\innprod{\nabla_{x_i}\phi(x_1^{k+1},\ldots,x_{i-1}^{k+1},x_i^{k},\ldots,x_q^{k})}{x-x_i^k}+\frac{1}{\gamma_{i,k}}\D_{h_1}(x,x_i^k)+f_i(x)}
	\end{equation*}
\State\label{state:bpalmk1}%
	$k= k+1$~ and go to \Cref{state:bpalmXk1}.%
\end{algorithmic}
\label{alg:gbpalm}
\end{algorithm*}%
%%%%%%%%%%%%%%%%%

